The complex geometry of Teichm\"uller spaces and bounded symmetric domains

We study isometric maps between Teichm\"uller spaces and bounded symmetric domains in their intrinsic Kobayashi metric. From a complex analytic perspective, these two important classes of geometric spaces have several features in common but also exhibit many differences. The focus here is on recent results proved by the author; we give a list of open questions at the end. Paper based on plenary talk presented to the 6th Ahlfors-Bers Colloquium at Yale, 23-26 October 2014.

==> bsds.tex <==
% ----------------------------------------------------------------
\addtocontents{toc}{\protect\setcounter{tocdepth}{1}}

% ----------------------------------------------------------------
\section{Symmetric spaces vs Teichm\"uller spaces}\label{sec:bsds}
% ----------------------------------------------------------------
Let $\T_{g,n}\subset\C^{3g-3+n}$ be a Teichm\"uller space and
$\mathcal{B}\subset\C^N$ a bounded symmetric domain equipped with their
\textit{Kobayashi} metrics. In this section, we complete the proof of
the following theorem.
\begin{thm}\label{thm:bsds}
  Let $\mathcal{B}\subset\C^{N}$ be a bounded symmetric domain and $\T_{g,n}$ be
  a Teichm\"uller space with $\text{dim}_{\C}\mathcal{B},\text{dim}_{\C}\T_{g,n}
  \geq 2$. There are no holomorphic isometric immersions \[\mathcal{B}
  \xhookrightarrow{~~~f~~~} \T_{g,n} \quad \text{or} \quad \T_{g,n}
  \xhookrightarrow{~~~f~~~} \mathcal{B}\] such that $df$ is an isometry for the
  Kobayashi norms on tangent spaces.~\\
\end{thm}
\begin{remarks}~\\
  1. Torelli maps (associating to a marked Riemann surface the
  Jacobians of its finite covers) give rise to holomorphic maps
  $\T_{g,n} \xhookrightarrow{~~~\mathcal{T}~~~} \mathcal{H}_h$ into
  bounded symmetric domains (Siegel spaces). It is known that these
  maps are not isometric for the Kobayashi metric in most
  directions.~\cite{McMullen:covs}~\\
  2. For a similar result about holomorphic isometric submersions
  see~\cite{Antonakoudis:birational}.
\end{remarks}
% ----------------------------------------------------------------
% \begin{thm}\label{thm:bsds:dual}
%   Let $\mathcal{B}$ and $\T_{g,n}$ be as in Theorem~\ref{thm:bsds}. There are no
%   holomorphic isometric submersions \[\mathcal{B} \xtwoheadrightarrow{g}
%   \T_{g,n} \quad \text{or} \quad \T_{g,n}\xtwoheadrightarrow{g} \mathcal{B}\]
%   such that $dg^{*}$ is an isometry for the \textit{dual} Kobayashi
%   norms on cotangent spaces.
% \end{thm}
% ----------------------------------------------------------------
% \restate{thm-bsd-conv} { Hello }
% ----------------------------------------------------------------
\subsection*{Outline of the proofs}
The proof that $\mathcal{B} \not\hookrightarrow \T_{g,n}$ follows from
Theorem~\ref{thm:balls} (rank one) and a classical application of
Sullivan's rigidity theorem (higher rank). The new ingredient we
introduce in this section is a comparison of the \textit{roughness} of
Kobayashi metric for bounded symmetric domains and Teichm\"uller
spaces, which we will use to prove that $\T_{g,n} \not\hookrightarrow \mathcal{B}$ 
\qed ~\\

\subsection*{Preliminaries on symmetric spaces}~\\
We give a quick review of the main features of symmetric spaces, from
a complex analysis perspective, which we use in the proof. We refer
to~\cite{Helgason:book:dglgss},~\cite{Satake:book:symmetric} for more
details.

Let $\mathcal{B} \subset \mathbb{C}^N$ be a bounded symmetric domain
and $p\in \mathcal{B}$. There is a \textit{unique}, up to
post-composition with a linear map, holomorphic embedding
$\mathcal{B}\xhookrightarrow{~~i~~}\C^N$ such that
$i(\mathcal{B}) \subset \C^N$ is a \textit{strictly convex} circular
domain with $i(p)= 0 \in \C^N$, which we refer to as the
Harish-Chandra realization of $\mathcal{B}$ centered at
$p\in \mathcal{B}$.

It is known that the Harish-Chandra realization of
$\mathcal{B}\subset \C^N$ has the following useful description. There
is a finite dimensional linear subspace
$V_{\mathcal{B}} \subset M_{n,m}(\C)$, of the space of complex
$n \times m$ matrices, such that
$\mathcal{B}\cong \{~~V \in V_{\mathcal{B}} ~~|~~ ||V||_{\mathcal{B}}
< 1~~ \}$
is the unit ball for the operator norm on $V_{\mathcal{B}}$, where
$||V||_{\mathcal{B}} = \text{sup}_{||\xi||_2 =1} ||V(\xi)||_2$, for
$V \in M_{n,m}(\C)$. We note that there is a natural identification
$T_{p}\mathcal{B} \cong V_{\mathcal{B}}\cong \C^N$.~\cite{Satake:book:symmetric}

The Kobayashi norm on $T_{p}\mathcal{B}\cong V_{\mathcal{B}}$
coincides with the operator norm $||V||_\mathcal{B}$, for
$V\in V_{\mathcal{B}} \subset M_{n,m}(\C)$ and the Kobayashi distance
from the origin is given by the formula
$d_\mathcal{B}(0,V)=\frac{1}{2}\log(\frac{1+||V||_\mathcal{B}}{1-||V||_\mathcal{B}})$,
for $V \in \mathcal{B}$.~\cite{Kubota:sym}~\\

\subsection*{Roughness of the Kobayashi metric}~\\
The following proposition describes the roughness of the Kobayashi
distance for bounded symmetric domains.

\begin{prop}\label{prop:bsd}
  Let $V: (-1,1) \rightarrow \mathcal{B}$ be a real-analytic path with
  $V(0)\neq p$. There is an integer $K >0$ and an $\epsilon >0 $ such
  that  $d_{\mathcal{B}}(p,V(\cdot)): [0,\epsilon)\rightarrow \mathcal{B}$
  is a real-analytic function of $t^{1/K}$ for $t \in [0,\epsilon)$.
\end{prop}
% ----------------------------------------------------------------
% \textit{dual} Kobayashi norm $T_{0}^{*}\mathcal{B} \cong V^{*}$
% coincides with the trace-class norm.
% ----------------------------------------------------------------
\begin{proof}
  Let
  $\mathcal{B} = \{~~||V||_{\mathcal{B}} < 1~~\}\subset
  V_{\mathcal{B}} \subset M_{n,m}(\C)$
  be the Harish-Chandra realization of $\mathcal{B}$ centered at $p$.
  For each $t\in (-1,1)$, we denote by $\lambda_i(t)$, for
  $i=1, \ldots, n$, the eigenvalues of the (positive) square matrix
  $V(t)^{*}V(t)$, counted with multiplicities, where $V^{*}$ denotes
  the Hermitian adjoint of $V$.

  The eigenvalues of $V(t)^{*}V(t)$ are the zeros of a polynomial, the
  coefficients of which are real-analytic functions of $t\in (-1,1)$.
  Therefore, the points $(t,\lambda_i (t)) \in \C^2$ for
  $i=1, \ldots, n$ and $t\in (-1,1)$ are contained in an algebraic
  curve $C= \{~~(t,\lambda) \in \C^2 ~~|~~ P(t,\lambda)=0~~\}$, which
  is equipped with a finite-degree branched covering map to
  $\mathbb{C}$ given by $(t,\lambda) \mapsto t$, for  $(t,\lambda) \in C$.

  Since the operator norm is given by the formula
  $|| V(t) ||_\mathcal{B} = \sup \{| \lambda_i (t)|^{1/2}\}_{i=1}^n$,
  the proof of the proposition follows by considering the Puiseux
  series expansion for $\lambda_i(t)$'s and the formula
  $d_\mathcal{B}(0,V(t))=\frac{1}{2}\log(\frac{1+||V(t)||_\mathcal{B}}{1-||V(t)||_\mathcal{B}})$.
% ----------------------------------------------------------------
  % Let $\mathcal{B} \subset \mathbb{C}$ be the union of the branching locus and
  % the image of the singular locus of $C$. Since $\mathcal{B}$ is discrete we can
  % find a small open disk $U$ around $0$, so that $\mathcal{B} \cap U \subset
  % \{0\}$. In particular the curve $C$ is smooth over $U\setminus
  % \{0\}$. The lemma follows by considering the Puiseux expansions of
  % the $\lambda$-branches over $t \in U$ and observing that for
  % sufficiently small positive real values of $t$ one of the solutions
  % will have maximal modulus $|\lambda_i(t)|$.
% ----------------------------------------------------------------
\end{proof}
% ----------------------------------------------------------------
% After choosing a basis, we can identify the dual of $V$ with $V$
% itself, and the dual operator norm with the trace-class norm on
% $V$. For $v \in V$ the trace-class norm equals $||v|| = Tr(|v|)$,
% where $|v|$ is the unique positive square root of the self-adjoint
% matrix $v^{*} v$. In particular we see that $||v|| = \sum_i |\lambda_i
% (v)|^{1/2}$, where $\lambda_i(v)$ are the eigenvalues of the matrix
% $v^{*}v$.
% ----------------------------------------------------------------
% Consider any two non-zero vectors $v$ and $w$ in $V$ and the function
% $f : t \mapsto Tr(|v+t\cdot w|)$. Arguing as in the lemma in section
% 2, we can find $\epsilon > 0$ small enough such that for $t \in [0,
% \epsilon)$ we can write $f(t)$ are a power series in $t^{1/k}$, for
% some positive integer $k$.
% ----------------------------------------------------------------
% \subsection*{Symmetric domains in dimension one and two}
% When $\text{dim}_{\C}\mathcal{B}=1$, we have $\mathcal{B} \cong \mathbb{CH}^1$; we recall
% that $\mathbb{CH}^1$ is the unit disk $\Delta \subset \C$ equipped
% with the Poincar\'e metric of constant curvature -4. When
% $\text{dim}_{\C}\mathcal{B}=2$, up to holomorphic isomorphism, we have that
% either $\mathcal{B} \cong \mathbb{CH}^2$ or
% $\mathcal{B} \cong \mathbb{CH}^1 \times \mathbb{CH}^1$.
% ----------------------------------------------------------------
% The Kobayashi metric on
% $\mathbb{CH}^2\cong\{~~(z,w)~~ | ~~ |z|^2 + |w|^2 < 1~~ \} \subset
% \C^2$
% coincides with the unique invariant Ka\"ehler metric with constant
% holomorphic curvature -4. In particular,
% $||\xi||_{\mathbb{CH}^2} = ||\xi||_2=\sqrt{|\xi_1|^2+|\xi_2|^2} $ for
% $\xi=(\xi_1,\xi_2) \in T_{(0,0)}\mathbb{CH}^2 \cong \C^2$.
% ----------------------------------------------------------------
% The Kobayashi metric on
% $\mathbb{CH}^1 \times \mathbb{CH}^1 \subset \C^2$ coincides with the
% sup-metric
% $||\xi||_{\mathbb{CH}^1\times\mathbb{CH}^1} = ||\xi||_{\infty} =
% \sup\{|\xi_1|,|\xi_2|\}$
% for
% $\xi=(\xi_1,\xi_2)\in T_{(0,0)}(\mathbb{CH}^1\times\mathbb{CH}^1)
% \cong \C^2$.
% We also note that the \textit{dual} Kobayashi metric is given by
% $||\phi||_{\mathbb{CH}^1\times\mathbb{CH}^1}=||\phi||_{1}=|\phi_{1}|+|\phi_{2}|$
% for
% $\phi=(\phi_1,\phi_2) \in
% T_{(0,0)}^{*}(\mathbb{CH}^1\times\mathbb{CH}^1) \cong
% \C^2$.~\cite{Kobayashi:book:hyperbolic}
% ----------------------------------------------------------------
% It is known that, when $\text{dim}_{\C}\mathcal{B} \geq 2$, there are
% holomorphic maps $f$ and $g$ such that: Either,
% \begin{equation}\label{eq:rank1}
%   \mathbb{CH}^2 \xhookrightarrow{~~~~f~~~~} \mathcal{B} \xtwoheadrightarrow{g} \mathbb{CH}^2 \qquad\text{and}\quad g\circ f = \text{id}_{\mathbb{CH}^2}
% \end{equation}
% Or,
% \begin{equation}\label{eq:rank2}
%   \mathbb{CH}^1\times\mathbb{CH}^1 \xhookrightarrow{~~~~f~~~~} \mathcal{B} \xtwoheadrightarrow{g} \mathbb{CH}^1\times\mathbb{CH}^1 \qquad\text{and}\quad g\circ f = \text{id}_{\mathbb{CH}^1\times\mathbb{CH}^1}
% \end{equation}
% %such that $g\circ f = \text{id}_{\mathbb{CH}^1\times\mathbb{CH}^1}$.
% ----------------------------------------------------------------
% \textit{We note that, in both cases, $df$ and $dg^{*}$ are isometries
%   for the Kobayashi norm on tangent spaces and the dual Kobayashi norm
%   on co-tangent spaces, respectively.}
% ----------------------------------------------------------------
% \subsection*{Rank and polydisks} 
% Let $\mathcal{B} \subset \mathbb{C}^N$ be a bounded symmetric domain and
% denote by
% $\Delta^N = \{~z=(z_{1}, \ldots,
% z_{N})~:~||z||_{\infty}=\text{sup}_{i=1}^{N}\{|z_{i}|\} < 1 ~\}$
% the unit polydisk in $\C^N$.
%
% It is known that there is a maximal integer $r$, the \textit{rank}
% of $\mathcal{B}$, with the following
% property~\cite{Kobayashi:book:hyperbolic}: For every point $p \in \mathcal{B}$
% there is an embedding $\mathcal{B}\subset\C^N$ that sends $p$ to
% $0\in \mathbb{C}^N$ and such that
% $\Delta^r \subset \mathcal{B} \subset \Delta^N$ where
% $\Delta^r = \{ z_{r+1} = \ldots = z_{N}=0\} \cap\Delta^N$.
% ----------------------------------------------------------------

The roughness of the Kobayashi metric for Teichm\"uller spaces is
described by the following two theorems of M.~Rees.
\begin{thm}(\cite{Rees:distance:c2}; M. Rees)\label{thm:c2} 
  The Teichm\"uller distance
  $d_{\T_{g,n}} : \T_{g,n}\times\T_{g,n} \rightarrow \R_{\geq 0}$ is
  $C^2$-smooth on the complement of the diagonal
  $d_{\T_{g,n}}^{-1}(0)$.
\end{thm}
\begin{thm}(\cite{Rees:distance:notc2}; M. Rees)\label{thm:notc2}
  When $\text{dim}_{\C}\T_{g,n} \geq 2$, the Teichm\"uller distance
  $d_{\T_{g,n}} : \T_{g,n}\times\T_{g,n} \rightarrow \R_{\geq 0}$ is
  \textit{not} $C^{2+\epsilon}$ for any $\epsilon>0$.

  Moreover, let $X,Y \in \T_{g,n}$ be two distinct points connected by
  a (real) Teichm\"uller geodesic which is generated by a quadratic
  differential $q\in Q_1(X)$, with either a zero of order two or
  number of poles less than $n$. There is a real analytic path
  $X(t):(-1,1)\rightarrow \T_{g,n}$ with $X(0)=X$ such that the
  distance $d_{\T_{g,n}}(X(t),Y)$ is not $C^{2+h}$-smooth at $t=0$,
  for every gauge function $h(t)$ with $\lim_{t \rightarrow 0}
  \frac{h(t)}{1/log(1/|t|)} = 0$.~\\
\end{thm}

\subsection*{Proof of Theorem~\ref{thm:bsds}}~\\
% ----------------------------------------------------------------

Let $\mathcal{B}\subset\C^{N}$ be a bounded symmetric domain and
$\T_{g,n}$ a Teichm\"uller space with
$\text{dim}_{\C}\mathcal{B},\text{dim}_{\C}\T_{g,n} \geq 2$. Using the
fact that bounded symmetric domains and Teichm\"uller spaces contain
holomorphic isometric copies of $\mathbb{CH}^1$ through every point
and complex direction, and a theorem of
Slodkowski~\cite{Slodkowski:motions},~\cite{Earle:Markovic:isometries},
we deduce that any holomophic map $f$ between $\mathcal{B}$ and
$\T_{g,n}$ which is an isometry for the Kobayashi norms on tangent
spaces would be totally-geodesic and would therefore preserve the
Kobayashi distance for pairs of points.~\\

\noindent\textbf{($\mathcal{B} \not\hookrightarrow \T_{g,n}$)}~\\

Theorem~\ref{thm:balls} shows that there is no holomorphic isometry
$f: \mathbb{CH}^2 \rightarrow \T_{g,n}$. Moreover, an application of
Sullivan's rigidity theorem (see ~\cite{Tanigawa:holomap} for a
precise statement) shows that there is no proper holomorphic map
$f: \mathbb{CH}^1 \times \mathbb{CH}^1 \rightarrow \T_{g,n}$, hence
neither is such a holomorphic map that is an isometry.

However, for every bounded symmetric domain $\mathcal{B}$ with
$\text{dim}_{\C}\mathcal{B} \geq 2$ there is either a holomorphic
totally-geodesic isometry $\mathbb{CH}^2 \hookrightarrow \mathcal{B}$
(rank one) or a holomorphic totally-geodesic isometry
$\mathbb{CH}^1\times \mathbb{CH}^1 \hookrightarrow \mathcal{B}$
(higher rank).~\cite{Kobayashi:book:metric} We conclude that there is
no holomorphic isometric immersion $f: \mathcal{B} \hookrightarrow \T_{g,n}$.~\\
% ----------------------------------------------------------------

\noindent\textbf{($\T_{g,n} \not\hookrightarrow \mathcal{B}$)}~\\

Let $f: \T_{g,n} \hookrightarrow \mathcal{B}$ be a holomorphic
isometric immersion. Since $\text{dim}_{\mathbb{C}}\T_{g,n} \geq 2$,
we can choose two distinct points $X,Y \in \T_{g,n}$ as described in
Theorem~\ref{thm:notc2}; hence there is a real analytic path
$X(t):(-1,1)\rightarrow \T_{g,n}$ with $X(0)=X$ such that the
Teichm\"uller distance $d_{\T_{g,n}}(X(t),Y)$ is not $C^{2+h}$-smooth
at $t=0$ for every gauge function $h(t)$ with
$\lim_{t \rightarrow 0} \frac{h(t)}{1/log(1/|t|)} = 0$.

Let $p=f(Y)\in \mathcal{B}$ and
$V(\cdot): (-1,1) \rightarrow \mathcal{B}$ be the real analytic path
given by $V(t) = f(X(t))$ for $t \in (-1,1)$. Theorem~\ref{thm:c2}
shows $d_{\mathcal{B}}(p,V(t))$ is $C^2$-smooth at $t=0$ and
Proposition~\ref{prop:bsd} shows that it is real analytic in
$t^{1/K}$, for some fixed integer $K>0$, for all sufficiently small
$t \geq 0$. Therefore, it follows that $d_{\T_{g,n}}(X(t),Y)$ is
$C^{2+\frac{1}{K}}$-smooth, but this contradicts the choice of the
path $X(t) \in \T_{g,n}$, given by Theorem~\ref{thm:notc2}, by
considering the gauge function $h(t)= t^{1/K}$ for $t \geq 0$. We
conclude that there is no holomorphic isometric immersion
$f: \T_{g,n} \hookrightarrow \mathcal{B}$.\qed
% ----------------------------------------------------------------

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

% ----------------------------------------------------------------

